The connection between halo concentrations and assembly histories: a probe of gravity?

We use two high resolution N-body simulations, one assuming general relativity and the other the Hu-Sawicki form of $f\left(R\right)$ gravity with $\vert \bar{f}_{R} \vert = 10^{-6}$, to investigate the concentration--formation time relation of dark matter haloes. We stack haloes in logarithmically spaced mass bins to fit median density profiles and extract median formation times. At fixed mass, haloes in modified gravity are more concentrated than those in GR, especially at low masses and at low redshift, and do not follow the concentration--formation time relation seen in GR. We assess the sensitivity of the relation to how concentration and formation time are defined, as well as to the segregation of the halo population by the amount of gravitational screening. We find a clear difference between halo concentrations and assembly histories displayed in modified gravity and those in GR. Existing models for the mass--concentration--redshift relation that have gained success in cold and warm dark matter models require revision in $f\left(R\right)$ gravity.

==> tags <==
!_TAG_FILE_FORMAT	2	/extended format; --format=1 will not append ;" to lines/
!_TAG_FILE_SORTED	1	/0=unsorted, 1=sorted, 2=foldcase/
!_TAG_OUTPUT_MODE	u-ctags	/u-ctags or e-ctags/
!_TAG_PROGRAM_AUTHOR	Universal Ctags Team	//
!_TAG_PROGRAM_NAME	Universal Ctags	/Derived from Exuberant Ctags/
!_TAG_PROGRAM_URL	https://ctags.io/	/official site/
!_TAG_PROGRAM_VERSION	0.0.0	/11ee721/
$\\fR$ gravity	oleskiewicz2019a.tex	/^\\subsection{$\\fR$ gravity}\\label{sec:fr}$/;"	u	section:Theory
.dot.pdf	makefile	/^.dot.pdf:$/;"	t
.tex.pdf	makefile	/^.tex.pdf:$/;"	t
Acknowledgements	oleskiewicz2019a.tex	/^\\section*{Acknowledgements}$/;"	s
Calculating halo formation times	oleskiewicz2019a.tex	/^\\subsection{Calculating halo formation times}\\label{sec:cmh}$/;"	u	section:Results
Conclusions	oleskiewicz2019a.tex	/^\\section{Conclusions}\\label{sec:conclusions}$/;"	s
Einasto profile	oleskiewicz2019a.tex	/^\\section{Einasto profile}\\label{sec:einasto}$/;"	s
Environmental screening	oleskiewicz2019a.tex	/^\\subsection{Environmental screening}\\label{sec:dnf}$/;"	u	section:Theory
Filtering \\& binning	oleskiewicz2019a.tex	/^\\subsection{Filtering \\& binning}\\label{sec:filter}$/;"	u	section:Results
Fitting mass profiles	oleskiewicz2019a.tex	/^\\subsection{Fitting mass profiles}\\label{sec:prof}$/;"	u	section:Results
Halo identification	oleskiewicz2019a.tex	/^\\subsection{Halo identification}\\label{sec:hbt}$/;"	u	section:Theory
Introduction	oleskiewicz2019a.tex	/^\\section{Introduction}\\label{sec:intro}$/;"	s
Mass-Concentration-Redshift relation	oleskiewicz2019a.tex	/^\\subsection{Mass-Concentration-Redshift relation}\\label{sec:cmz}$/;"	u	section:Theory
Merger trees	oleskiewicz2019a.tex	/^\\subsection{Merger trees}\\label{sec:mt}$/;"	u	section:Theory
Results	oleskiewicz2019a.tex	/^\\section{Results}\\label{sec:results}$/;"	s
Sensitivity to variation of model parameters	oleskiewicz2019a.tex	/^\\subsection{Sensitivity to variation of model parameters}\\label{sec:params}$/;"	u	section:Results
Separation of haloes by screening	oleskiewicz2019a.tex	/^\\subsection{Separation of haloes by screening}\\label{sec:sep_dnf}$/;"	u	section:Results
TC	makefile	/^TC      = tectonic$/;"	m
TCFLAGS	makefile	/^TCFLAGS = -C -k -c minimal$/;"	m
The density--density relation	oleskiewicz2019a.tex	/^\\subsection{The density--density relation}\\label{sec:rhorho}$/;"	u	section:Results
Theory	oleskiewicz2019a.tex	/^\\section{Theory}\\label{sec:theory}$/;"	s
akaike1974	oleskiewicz2019a.bib	/^@article{akaike1974,$/;"	b
all	makefile	/^all: oleskiewicz2019a.pdf$/;"	t
angel2016	oleskiewicz2019a.bib	/^@article{angel2016,$/;"	b
arnold2016	oleskiewicz2019a.bib	/^@article{arnold2016,$/;"	b
arnold2018	oleskiewicz2019a.bib	/^@article{arnold2018,$/;"	b
baugh2006a	oleskiewicz2019a.bib	/^@article{baugh2006a,$/;"	b
benson2018	oleskiewicz2019a.bib	/^@article{benson2018,$/;"	b
berry2011	oleskiewicz2019a.bib	/^@article{berry2011,$/;"	b
binney1987	oleskiewicz2019a.bib	/^@book{binney1987,$/;"	b
birkhoff1923	oleskiewicz2019a.bib	/^@book{birkhoff1923,$/;"	b
bond1991	oleskiewicz2019a.bib	/^@article{bond1991,$/;"	b
bose2015	oleskiewicz2019a.bib	/^@article{bose2015,$/;"	b
bose2016	oleskiewicz2019a.bib	/^@article{bose2016,$/;"	b
bose2017	oleskiewicz2019a.bib	/^@article{bose2017,$/;"	b
buchdahl1970	oleskiewicz2019a.bib	/^@article{buchdahl1970,$/;"	b
bullock2001	oleskiewicz2019a.bib	/^@article{bullock2001,$/;"	b
carroll2001	oleskiewicz2019a.bib	/^@article{carroll2001,$/;"	b
carroll2004	oleskiewicz2019a.bib	/^@article{carroll2004,$/;"	b
cataneo2015	oleskiewicz2019a.bib	/^@article{cataneo2015,$/;"	b
child2018	oleskiewicz2019a.bib	/^@article{child2018,$/;"	b
clean	makefile	/^clean:$/;"	t
clifton2012	oleskiewicz2019a.bib	/^@article{clifton2012,$/;"	b
clifton2013	oleskiewicz2019a.bib	/^@article{clifton2013,$/;"	b
cole1996	oleskiewicz2019a.bib	/^@article{cole1996,$/;"	b
cole2000	oleskiewicz2019a.bib	/^@article{cole2000,$/;"	b
cole2008	oleskiewicz2019a.bib	/^@article{cole2008,$/;"	b
correa2015	oleskiewicz2019a.bib	/^@article{correa2015,$/;"	b
davis1985	oleskiewicz2019a.bib	/^@article{davis1985,$/;"	b
diemer2015	oleskiewicz2019a.bib	/^@article{diemer2015,$/;"	b
diemer2019	oleskiewicz2019a.bib	/^@article{diemer2019,$/;"	b
duffy2008	oleskiewicz2019a.bib	/^@article{duffy2008,$/;"	b
dziak2012	oleskiewicz2019a.bib	/^@article{dziak2012,$/;"	b
einasto1965	oleskiewicz2019a.bib	/^@inproceedings{einasto1965,$/;"	b
eqn:F	oleskiewicz2019a.tex	/^\\begin{equation} \\label{eqn:F}$/;"	l
eqn:chi	oleskiewicz2019a.tex	/^\\begin{equation}\\label{eqn:chi}$/;"	l
eqn:d_off	oleskiewicz2019a.tex	/^\\begin{equation}\\label{eqn:d_off}$/;"	l
eqn:delta_c	oleskiewicz2019a.tex	/^\\begin{equation}\\label{eqn:delta_c}$/;"	l
eqn:eps	oleskiewicz2019a.tex	/^\\begin{equation}\\label{eqn:eps}$/;"	l
eqn:fr	oleskiewicz2019a.tex	/^\\begin{equation}\\label{eqn:fr}$/;"	l
eqn:hs	oleskiewicz2019a.tex	/^\\begin{equation}\\label{eqn:hs}$/;"	l
eqn:nfw	oleskiewicz2019a.tex	/^\\begin{equation}\\label{eqn:nfw}$/;"	l
eqn:poisson	oleskiewicz2019a.tex	/^\\begin{equation}\\label{eqn:poisson}$/;"	l
eqn:r_min	oleskiewicz2019a.tex	/^	      \\begin{equation}\\label{eqn:r_min}$/;"	l
eqn:z_form	oleskiewicz2019a.tex	/^\\begin{equation}\\label{eqn:z_form}$/;"	l
fig:cmh	oleskiewicz2019a.tex	/^	\\label{fig:cmh}$/;"	l
fig:dnf	oleskiewicz2019a.tex	/^	\\label{fig:dnf}$/;"	l
fig:prof	oleskiewicz2019a.tex	/^	\\label{fig:prof}$/;"	l
fig:rhorho_cut	oleskiewicz2019a.tex	/^	\\label{fig:rhorho_cut}$/;"	l
fig:rhorho_mstar	oleskiewicz2019a.tex	/^	\\label{fig:rhorho_mstar}$/;"	l
fig:rhorho_var_NFW_f	oleskiewicz2019a.tex	/^	\\label{fig:rhorho_var_NFW_f}$/;"	l
fig:rhorho_var_rs_f	oleskiewicz2019a.tex	/^	\\label{fig:rhorho_var_rs_f}$/;"	l
fig:rhorho_z	oleskiewicz2019a.tex	/^	\\label{fig:rhorho_z}$/;"	l
fig:tree	oleskiewicz2019a.tex	/^	\\label{fig:tree}$/;"	l
firstpage	oleskiewicz2019a.tex	/^\\label{firstpage}$/;"	l
frenk1985	oleskiewicz2019a.bib	/^@article{frenk1985,$/;"	b
fukushige2001	oleskiewicz2019a.bib	/^@article{fukushige2001,$/;"	b
gao2008	oleskiewicz2019a.bib	/^@article{gao2008,$/;"	b
gunn1972	oleskiewicz2019a.bib	/^@article{gunn1972,$/;"	b
haas2012	oleskiewicz2019a.bib	/^@article{haas2012,$/;"	b
han2012	oleskiewicz2019a.bib	/^@article{han2012,$/;"	b
han2018	oleskiewicz2019a.bib	/^@article{han2018,$/;"	b
he2018	oleskiewicz2019a.bib	/^@article{he2018,$/;"	b
hellwing2013	oleskiewicz2019a.bib	/^@article{hellwing2013,$/;"	b
hellwing2016	oleskiewicz2019a.bib	/^@article{hellwing2016,$/;"	b
hernandez-aguayo2018	oleskiewicz2019a.bib	/^@article{hernandez-aguayo2018,$/;"	b
hernquist1990	oleskiewicz2019a.bib	/^@article{hernquist1990,$/;"	b
hinshaw2013	oleskiewicz2019a.bib	/^@article{hinshaw2013,$/;"	b
hu2007	oleskiewicz2019a.bib	/^@article{hu2007,$/;"	b
jennings2012	oleskiewicz2019a.bib	/^@article{jennings2012,$/;"	b
jiang2013	oleskiewicz2019a.bib	/^@article{jiang2013,$/;"	b
joyce2015	oleskiewicz2019a.bib	/^@article{joyce2015,$/;"	b
kauffmann1993	oleskiewicz2019a.bib	/^@article{kauffmann1993,$/;"	b
khoury2004	oleskiewicz2019a.bib	/^@article{khoury2004,$/;"	b
klypin2016	oleskiewicz2019a.bib	/^@article{klypin2016,$/;"	b
koyama2016	oleskiewicz2019a.bib	/^@article{koyama2016,$/;"	b
lacerna2017	oleskiewicz2019a.bib	/^@article{lacerna2017,$/;"	b
lacey1993	oleskiewicz2019a.bib	/^@article{lacey1993,$/;"	b
lacey2015	oleskiewicz2019a.bib	/^@article{lacey2015,$/;"	b
lagos2011	oleskiewicz2019a.bib	/^@article{lagos2011,$/;"	b
lastpage	oleskiewicz2019a.tex	/^\\label{lastpage}$/;"	l
lee2014	oleskiewicz2019a.bib	/^@article{lee2014,$/;"	b
li2011	oleskiewicz2019a.bib	/^@article{li2011,$/;"	b
li2012c	oleskiewicz2019a.bib	/^@article{li2012c,$/;"	b
li2013	oleskiewicz2019a.bib	/^@article{li2013,$/;"	b
liu2016	oleskiewicz2019a.bib	/^@article{liu2016,$/;"	b
lombriser2014a	oleskiewicz2019a.bib	/^@article{lombriser2014a,$/;"	b
lombriser2014b	oleskiewicz2019a.bib	/^@article{lombriser2014b,$/;"	b
ludlow2010	oleskiewicz2019a.bib	/^@article{ludlow2010,$/;"	b
ludlow2013	oleskiewicz2019a.bib	/^@article{ludlow2013,$/;"	b
ludlow2014a	oleskiewicz2019a.bib	/^@article{ludlow2014a,$/;"	b
ludlow2014b	oleskiewicz2019a.bib	/^@article{ludlow2014b,$/;"	b
ludlow2016	oleskiewicz2019a.bib	/^@article{ludlow2016,$/;"	b
ludlow2018	oleskiewicz2019a.bib	/^@article{ludlow2018,$/;"	b
maccio2007	oleskiewicz2019a.bib	/^@article{maccio2007,$/;"	b
maccio2008	oleskiewicz2019a.bib	/^@article{maccio2008,$/;"	b
maccio2013	oleskiewicz2019a.bib	/^@article{maccio2013,$/;"	b
martino2009	oleskiewicz2019a.bib	/^@article{martino2009,$/;"	b
massey2015	oleskiewicz2019a.bib	/^@article{massey2015,$/;"	b
mitchell2019	oleskiewicz2019a.bib	/^@article{mitchell2019,$/;"	b
mo2010	oleskiewicz2019a.bib	/^@book{mo2010,$/;"	b
moore1998	oleskiewicz2019a.bib	/^@article{moore1998,$/;"	b
mota2007	oleskiewicz2019a.bib	/^@article{mota2007,$/;"	b
navarro1996	oleskiewicz2019a.bib	/^@article{navarro1996,$/;"	b
navarro1997	oleskiewicz2019a.bib	/^@article{navarro1997,$/;"	b
neistein2006	oleskiewicz2019a.bib	/^@article{neistein2006,$/;"	b
neto2007	oleskiewicz2019a.bib	/^@article{neto2007,$/;"	b
nsync	makefile	/^nsync:$/;"	t
nunes2017	oleskiewicz2019a.bib	/^@article{nunes2017,$/;"	b
oleskiewicz2019a.pdf	dep.mk	/^oleskiewicz2019a.pdf : oleskiewicz2019a.tex \\$/;"	t
oleskiewicz2019a_src	oleskiewicz2019a.bib	/^@article{oleskiewicz2019a_src,$/;"	b
parkinson2007	oleskiewicz2019a.bib	/^@article{parkinson2007,$/;"	b
peebles1980	oleskiewicz2019a.bib	/^@book{peebles1980,$/;"	b
planckcollaboration2016	oleskiewicz2019a.bib	/^@article{planckcollaboration2016,$/;"	b
poveda-ruiz2016	oleskiewicz2019a.bib	/^@article{poveda-ruiz2016,$/;"	b
power2003	oleskiewicz2019a.bib	/^@article{power2003,$/;"	b
prada2012	oleskiewicz2019a.bib	/^@article{prada2012,$/;"	b
press1974	oleskiewicz2019a.bib	/^@article{press1974,$/;"	b
robertson2017	oleskiewicz2019a.bib	/^@article{robertson2017,$/;"	b
schmidt2009	oleskiewicz2019a.bib	/^@article{schmidt2009,$/;"	b
schwarz1978	oleskiewicz2019a.bib	/^@article{schwarz1978,$/;"	b
sec:cmh	oleskiewicz2019a.tex	/^\\subsection{Calculating halo formation times}\\label{sec:cmh}$/;"	l
sec:cmz	oleskiewicz2019a.tex	/^\\subsection{Mass-Concentration-Redshift relation}\\label{sec:cmz}$/;"	l
sec:conclusions	oleskiewicz2019a.tex	/^\\section{Conclusions}\\label{sec:conclusions}$/;"	l
sec:dnf	oleskiewicz2019a.tex	/^\\subsection{Environmental screening}\\label{sec:dnf}$/;"	l
sec:einasto	oleskiewicz2019a.tex	/^\\section{Einasto profile}\\label{sec:einasto}$/;"	l
sec:filter	oleskiewicz2019a.tex	/^\\subsection{Filtering \\& binning}\\label{sec:filter}$/;"	l
sec:fr	oleskiewicz2019a.tex	/^\\subsection{$\\fR$ gravity}\\label{sec:fr}$/;"	l
sec:hbt	oleskiewicz2019a.tex	/^\\subsection{Halo identification}\\label{sec:hbt}$/;"	l
sec:intro	oleskiewicz2019a.tex	/^\\section{Introduction}\\label{sec:intro}$/;"	l
sec:mt	oleskiewicz2019a.tex	/^\\subsection{Merger trees}\\label{sec:mt}$/;"	l
sec:params	oleskiewicz2019a.tex	/^\\subsection{Sensitivity to variation of model parameters}\\label{sec:params}$/;"	l
sec:prof	oleskiewicz2019a.tex	/^\\subsection{Fitting mass profiles}\\label{sec:prof}$/;"	l
sec:results	oleskiewicz2019a.tex	/^\\section{Results}\\label{sec:results}$/;"	l
sec:rhorho	oleskiewicz2019a.tex	/^\\subsection{The density--density relation}\\label{sec:rhorho}$/;"	l
sec:sep_dnf	oleskiewicz2019a.tex	/^\\subsection{Separation of haloes by screening}\\label{sec:sep_dnf}$/;"	l
sec:theory	oleskiewicz2019a.tex	/^\\section{Theory}\\label{sec:theory}$/;"	l
sheth1999	oleskiewicz2019a.bib	/^@article{sheth1999,$/;"	b
shi2015	oleskiewicz2019a.bib	/^@article{shi2015,$/;"	b
shi2017	oleskiewicz2019a.bib	/^@article{shi2017,$/;"	b
somerville1999	oleskiewicz2019a.bib	/^@article{somerville1999,$/;"	b
springel2001	oleskiewicz2019a.bib	/^@article{springel2001,$/;"	b
springel2005b	oleskiewicz2019a.bib	/^@article{springel2005b,$/;"	b
sync	makefile	/^sync: clean$/;"	t
tbl:fit	oleskiewicz2019a.tex	/^	\\label{tbl:fit}$/;"	l
tbl:nbody	oleskiewicz2019a.tex	/^	\\label{tbl:nbody}$/;"	l
terukina2014	oleskiewicz2019a.bib	/^@article{terukina2014,$/;"	b
thomas2001	oleskiewicz2019a.bib	/^@article{thomas2001,$/;"	b
thomas2015	oleskiewicz2019a.bib	/^@article{thomas2015,$/;"	b
upadhye2013	oleskiewicz2019a.bib	/^@article{upadhye2013,$/;"	b
vainio2017	oleskiewicz2019a.bib	/^@article{vainio2017,$/;"	b
vandenbosch2013	oleskiewicz2019a.bib	/^@inproceedings{vandenbosch2013,$/;"	b
virgo2006	oleskiewicz2019a.bib	/^@article{virgo2006,$/;"	b
wechsler2002	oleskiewicz2019a.bib	/^@article{wechsler2002,$/;"	b
zhao2003	oleskiewicz2019a.bib	/^@article{zhao2003,$/;"	b
zhao2009	oleskiewicz2019a.bib	/^@article{zhao2009,$/;"	b
zhao2011	oleskiewicz2019a.bib	/^@article{zhao2011,$/;"	b
zuntz2010	oleskiewicz2019a.bib	/^@article{zuntz2010,$/;"	b

